Sage: Parallel Semi-Asymmetric Graph Algorithms for NVRAMs

Non-volatile main memory (NVRAM) technologies provide an attractive set of features for large-scale graph analytics, including byte-addressability, low idle power, and improved memory-density. NVRAM systems today have an order of magnitude more NVRAM than traditional memory (DRAM). NVRAM systems could therefore potentially allow very large graph problems to be solved on a single machine, at a modest cost. However, a significant challenge in achieving high performance is in accounting for the fact that NVRAM writes can be much more expensive than NVRAM reads. In this paper, we propose an approach to parallel graph analytics using the Parallel Semi-Asymmetric Model (PSAM), in which the graph is stored as a read-only data structure (in NVRAM), and the amount of mutable memory is kept proportional to the number of vertices. Similar to the popular semi-external and semi-streaming models for graph analytics, the PSAM approach assumes that the vertices of the graph fit in a fast read-write memory (DRAM), but the edges do not. In NVRAM systems, our approach eliminates writes to the NVRAM, among other benefits. To experimentally study this new setting, we develop Sage, a parallel semi-asymmetric graph engine with which we implement provably-efficient (and often work-optimal) PSAM algorithms for over a dozen fundamental graph problems. We experimentally study Sage using a 48-core machine on the largest publicly-available real-world graph (the Hyperlink Web graph with over 3.5 billion vertices and 128 billion edges) equipped with Optane DC Persistent Memory, and show that Sage outperforms the fastest prior systems designed for NVRAM. Importantly, we also show that Sage nearly matches the fastest prior systems running solely in DRAM, by effectively hiding the costs of repeatedly accessing NVRAM versus DRAM.

==> inputs/filtering-apx.tex <==
\section{Graph Filtering}\label{apx:filter}

In this section, we provide additional details on the algorithms used
to implement graph filter primitives and their work-depth bounds in
the \SAMabbrev{}. The algorithms use the parallel primitives
defined in Section~\ref{sec:prelims}.

\myparagraph{Graph Filter Algorithms}
We now describe our algorithms implementing primitives over the graph
filter structure, and analyze their costs. Our algorithms support both
uncompressed graphs, and graphs compressed using the parallel encoding
scheme from Ligra+~\cite{shun2015ligraplus}, and we describe any
encoding-specific changes required in what follows.

\emph{Creation.} To create a graph filter, the algorithm first
computes the number of blocks that each vertex requires, based on
\filterbs{}, and writes the space required per vertex into an array.
Next, it scans the array, and allocates the required $O(m)$ bits of
memory contiguously. It then initializes the blocks per-vertex, in
parallel, marking all edges as initially active (their corresponding
bit is set to 1). Finally, it allocates an array of per-vertex words
storing the initial degree, offset into the bitset structure
corresponding to the start of the vertex's blocks, and the number of
blocks for that vertex. Lastly, it marks each of the $n$ per-vertex
dirty bits to $\mathsf{false}$, as vertices are not initially marked
dirty. The overall work of the procedure is $O(m)$ and the overall
depth is $O(\log n + \filterbs{})$. If the user specifies that the
initially supplied predicate returns $\mathsf{false}$ for some edges,
the implementation calls \filteredges{} (described below), which runs
within the same work and depth bounds.

\emph{Packing.} Next, we describe the algorithm used to pack out the
edges incident to a vertex given a predicate $P$. The same algorithm
is used to implement both \filteredges{} and \emappack{}. The
algorithm first maps over all blocks currently incident to the vertex
in parallel. For each block, it finds all active bits in the block,
reads the edge corresponding to the active bit and applies the
predicate $P$. The algorithm unsets the bit if and only if the
predicate returns $\mathsf{false}$. If the bit for an edge $(u, v)$ is
unset, the algorithm marks the dirty bit for $v$ to true. Note that
for uncompressed graphs, the edge corresponding to an active bit can
be directly read, whereas for a compressed graph, the entire block may
have to be decoded to retrieve the value of a particular edge.

The algorithm also keeps track of how many bits are still active after
processing the entire block, and stores these per-block counts in an
array with size proportional to the number of blocks. Next, it
performs a reduction over this array to compute the number of blocks
with at least one active edge. For work-efficiency, if this value is less than a constant
fraction of the current number of blocks for this vertex, the algorithm filters
all blocks with no active elements, and packs the active blocks
contiguously in the same memory. This operation is implemented by
performing a parallel filter over the blocks. Next, the algorithm
updates the offsets for all blocks by performing a parallel scan.
Lastly, the algorithm updates the vertex degree and number of
currently active blocks incident to the vertex. The overall work done
is
$O(A \cdot (\filterbs{}/\log n) +  d_{\emph{active}}(v))$
and the depth is
$O(\log n + \filterbs{})$, where $A$ is the number of non-empty blocks
corresponding to $v$ and $d_{\emph{active}}(v)$ is the number of
active edges incident to vertex $v$. Note that the framework does not
expose this primitive directly to graph algorithms, since the number
of edges in the graph is not updated.

\emph{\filteredges{}.} The \filteredges{} primitive can be easily
implemented using the algorithm for packing a vertex above by packing
each vertex in parallel. The algorithm then returns the new degree of
the graph by reducing all vertex degrees. By summing over all calls to
the vertex packing primitive above, and accounting for the reduction
over $n$ vertices, the work is
$O(n + A\cdot (\filterbs{}/\log n) + |E_{active}|)$, and the depth is
$O(\log n + \filterbs{})$, where $A$ is the number of non-empty blocks in the graph and $E_{active}$ is the set
of active edges represented by the graph filter.

\emph{\emappack{}.} The \emappack{} primitive is implemented by
packing each vertex in the \vset{} in parallel. The overall work is
the sum of the work for packing out each vertex in the \vset{}, $S$,
which is $O(A\cdot \filterbs{}/\log n + \sum_{v\in
S}(1+d_{\emph{active}}(v)))$, and the depth is $O(\log n +
\filterbs{})$, where $A$ is the number of non-empty blocks
corresponding to all $v \in S$.

\emph{Vertex Primitives.} When calling vertex primitives on a graph
filter, such as accessing the degree of the vertex, or mapping over
its incident active edges, we first check whether the vertex is marked
dirty. If so, we pack it out using the algorithm described above
before performing the requested operation.

\myparagraph{Implementation and Optimizations}
Our routines were initially implemented by testing single bits at a
time when decoding a block for its active edges. However, if a block
is mostly empty, a large amount of CPU time is wasted checking bits
that are set to $0$. Instead, we use the \textsc{tzcnt} and \textsc{blsr} intrinsics that are provided on
modern x86 CPU architectures to accelerate block processing. Since
each block is logically divided into a number of machine words, we
consider processing a single machine word. If the word is non-zero, we
create a temporary copy of the word, and loop while this copy is
non-zero. In each iteration, we use \textsc{tzcnt} to find the index
of the next lowest bit, and clear the lowest bit using the
\textsc{blsr} instruction. Doing so allows us to process a block with
$q$ words and $k$ non-zero bits in $O(q + k)$ instructions.

We also implemented intersection primitives, which are used in our
triangle counting algorithm based on the decoding implementation
described above. For compressed graphs, since we may have to decode an
entire block, we first decompress the entire block and store it
locally in the iterator's memory. We then process the graph filter's
bits word-by-word using the intrinsic-based algorithm described above.

Finally, we avoid the use of dirty bits in the algorithms using the
graph filtering structure studied in this paper by supplying the
framework's primitives with a flag which informs the framework that
the algorithm will not operate on vertices which are not packed. By
avoiding using the dirty bits, our algorithms avoid an extra
random-write of a neighbor's dirty-bit when performing pack
operations, an a random-read to check a dirty-bit when performing
operations on vertices.



==> inputs/model-apx.tex <==
\section{Model Details}\label{sec:model-app}

In this section, we define the \defn{\SAM{}}, which borrows ideas from
the \SEM{} model~\cite{Abello2002,pearce2010multithreaded}, the \SSt{}
model~\cite{Muthukrishnan2005,feigenbaum2005graph}, the T-RAM
model~\cite{dhulipala18scalable}, and the
asymmetric nested-parallel (ANP) model~\cite{BBFGGMS16}.  We believe
that the new model captures the performance considerations in
designing graph algorithms on the existing systems based on NVRAMs.
similarities and differences compared to the previous models will be
discussed later in this section.

\subsection{\SAM{}}
The \SAM{} consists of an asymmetric \largemem{} with unbounded size that can hold the entire graph, and a symmetric \smallmem{} with $O(n)$ words of memory.
In a relaxed version, we allow the \smallmem{} size to store $O(n+m/\log n)$ words.
The \SAM{} has a set of \thread{}s that share both the \largemem{} and \smallmem{}.
Each \thread{} acts like a sequential RAM plus a \forkins{} instruction that forks two new child \thread{}s.
When a \thread{} performs a \forkins{}, the two child \thread{}s all start by running the next
instruction, and the original \thread{} is suspended until all the children terminate.
A computation starts with a single {root} \thread{} and finishes when that root \thread{} finishes.
This model supports what is often referred to as nested-parallelism.
This computational model is referred to as the T-RAM model or the binary-forking model.  More details are discussed in~\cite{dhulipala18scalable}.

We use the classic work-depth measure for the cost of algorithms on the \SAM{}.
Similar to the ANP model, we assume unit cost for a read or write to the \smallmem{}, and a read from the \largemem{}, both in the unit of a word.
A write to the \largemem{} has a cost of $\wcost{}$, which is the cost of a write relative to a read.
The overall \emph{work} $W$ of an algorithm is the cost for all memory accesses by all \thread{}s.
The \emph{depth} $D$ is the longest sequence of dependent instructions in this computation.
A work-stealing scheduler can execute such computation in $W/p+O(D)$ time with high probability on a PRAM with $p$ processors~\cite{BBFGGMS16}.

\subsection{Comparison to Existing Models}

\myparagraph{T-RAM and Binary-Forking Model}
The \SAM{} extends the memory in these models to two memories---the \smallmem{} resembles DRAM and the \largemem{} resembles NVRAM.

\myparagraph{Semi-External Memory Model}
The \SEM{} model~\cite{Abello2002} is a variant of the external-memory model~\cite{AggarwalV88} where there is a \smallmem{} that can hold the vertices but not the edges.
Compared to the \SAM{}, the \SEM{} does not account for the cost in accessing the \smallmem{} (DRAM), while we believe that for existing systems with NVRAMs, this cost is not negligible.
Second, the \SEM{} model has a parameter $B$ for the unit of data movement.
As opposed to external memories, NVRAMs support random access.
We decided to not use the parameter $B$ for ease of algorithm design and analysis.

\myparagraph{Semi-Streaming Model}
In the \SSt{} model~\cite{Muthukrishnan2005}, there is a memory size of $O(n \cdot \text{polylog}(n))$ bits
and algorithms can only read over the graph in a sequential streaming order (with possibly multiple passes). In contrast, the \SAM{} allows random access to the input graph
 because NVRAMs intrinsically support random access. Furthermore the \SAM{} allows writes to the \largemem{} with a higher cost.



==> inputs/primitives-apx.tex <==
\section{Parallel primitives}\label{apx:primitives}
The following parallel procedures are used in the remainder of the
Appendix.  \defn{Scan} takes as input an array $A$ of length $n$, an
associative binary operator $\oplus$, and an identity element $\bot$
such that $\bot \oplus x = x$ for any $x$, and returns the array
$(\bot, \bot \oplus A[0], \bot \oplus A[0] \oplus A[1], \ldots, \bot
\oplus_{i=0}^{n-2} A[i])$ as well as the overall sum, $\bot
\oplus_{i=0}^{n-1} A[i]$.  \defn{Reduce} takes an array $A$ and a
binary associative function $f$ and returns the sum of the elements in
$A$ with respect to $f$.  \defn{Filter} takes an array $A$ and a
predicate $f$ and returns a new array containing $a \in A$ for which
$f(a)$ is true, in the same order as in $A$.  If done in \smallmem{},
scan, reduce and filter can all be done in $O(n)$ work and $O(\log n)$
depth (assuming $\oplus$ and $f$ takes $O(1)$ work)~\cite{JaJa92}.


==> inputs/us_vs_memmode.tex <==
%\begin{tbox}
\begin{table}[t]
  \footnotesize
  \centering
%\scalebox{0.92}{
\setlength{\tabcolsep}{3pt}
\begin{tabular}[!t]{l|c|c|c|c}
%    \toprule
  \multicolumn{1}{c|}{\textbf{Problem}} & $\text{Gal}_{MM}$ & $\frac{\text{Gal}_{MM}}{\text{Us}}$ & $\text{Our}_{MM}$ & $\frac{\text{Our}_{MM}}{\text{Us}}$ \\
    \midrule
    BFS                    &35.2          & 2.88x &35.7   & 2.92x \\
    Weighted BFS           &---           & ---   &190    & 1.93x \\
    Bellman-Ford           &118           & 1.43x &149    & 1.81x \\
    1-Source Widest Path   &---           & ---   &89.8   & 1.15x \\
    1-Source Betweenness   &56.4          & 0.82x &148    & 2.16x \\
    $O(k)$-Spanner         &---           & ---   &124.8  & 2.26x \\
    LDD                    &---           & ---   &62.2   & 2.59x \\
    Connectivity           &76.0          & 2.09x &75.8   & 2.09x \\
    Spanning Forest        &---           & ---   &116    & 1.89x \\
    Biconnectivity         &---           & ---   &482    & 2.05x \\
    MIS                    &---           & ---   &98.8   & 2.24x \\
    Maximal Matching       &---           & ---   &455    & 2.74x \\
    Graph Coloring         &---           & ---   &216    & 0.90x \\
    Apx Set Cover          &---           & ---   &246    & 1.27x \\
    $k$-core               &---           & ---   &259    & 1.20x \\
    Apx Densest Subgraph   &---           & ---   &106    & 2.51x \\
    Triangle Counting      &---           & ---   &1665   & 0.47x \\
    PageRank Iteration     &---           & ---   &37.5   & 1.58x \\
    PageRank               &1706          & 2.12x &1318   & 1.59x \\
  \end{tabular}
%}
 % \par
%\vspace*{1em}
\caption{\small Parallel running time in seconds for Galois
  implementations using \memorymode{} (Gal-MM) and unmodified GBBS
  codes run using \memorymode{} (Our-MM) for the Hyperlink2012 graph.
  The columns (Gal-MM/Us) and (Our-MM/Us) provide the ratio of the
  Gal-MM and Our-MM times compared to our \nvm{} codes run using
  \appdirectmode{} for the same problem and graph. Note that the
  Gal-MM times are obtained using the directed version of the
  Hyperlink2012 graph.  The times reported for Galois are courtesy of
  the authors, who run on an identically configured machine, with 6TB
  of \nvm{}. We mark entries for problems that they do not report
  numbers for with ---. All of our experiments are run on a system with 375GB of
  DRAM, extended to 1.5TB of memory using \memorymode{}, and using 48
  cores with hyper-threading.}\label{table:usvsmemmode}
\end{table}
%\end{tbox}

